TrustRAG: An Information Assistant with Retrieval Augmented Generation

\Ac{RAG} has emerged as a crucial technique for enhancing large models with real-time and domain-specific knowledge. While numerous improvements and open-source tools have been proposed to refine the \ac{RAG} framework for accuracy, relatively little attention has been given to improving the trustworthiness of generated results. To address this gap, we introduce TrustRAG, a novel framework that enhances \ac{RAG} from three perspectives: indexing, retrieval, and generation. Specifically, in the indexing stage, we propose a semantic-enhanced chunking strategy that incorporates hierarchical indexing to supplement each chunk with contextual information, ensuring semantic completeness. In the retrieval stage, we introduce a utility-based filtering mechanism to identify high-quality information, supporting answer generation while reducing input length. In the generation stage, we propose fine-grained citation enhancement, which detects opinion-bearing sentences in responses and infers citation relationships at the sentence-level, thereby improving citation accuracy. We open-source the TrustRAG framework and provide a demonstration studio designed for excerpt-based question answering tasks \footnote{https://huggingface.co/spaces/golaxy/TrustRAG}. Based on these, we aim to help researchers: 1) systematically enhancing the trustworthiness of \ac{RAG} systems and (2) developing their own \ac{RAG} systems with more reliable outputs.

==> figures/library_dir.tex <==
\lstset{
    basicstyle=\ttfamily\small,
    breaklines=true,
    frame=single,
    caption={The TrustRAG Library},
    label=lst:directory_structure
}

\begin{lstlisting}
TrustRAG/
|--api
|  |--apps
|      |--config
|      |--core
|      |  |--citation
|      |  |--judge
|      |  |--parser
|      |  |--refiner
|      |  |--rerank
|      |  |--rewrite
|      |--handle
|      |  |--exception
|      |  |--response
|--docs
|--examples
|--notebooks
|--resources
|--tests
|--trustrag
|    |--applications
|    |--modules

\end{lstlisting}
% |    |  |--chunks
% |    |  |--citation
% |    |  |--clusters
% |    |  |--document
% |    |  |--engine
% |    |  |--generator
% |    |  |--judger
% |    |  |--postprocess
% |    |  |--processor
% |    |  |--prompt
% |    |  |--refiner
% |    |  |--reranker
% |    |  |--retrieval
% |    |  |--rewriter
